Cross-Modality High-Frequency Transformer for MR Image Super-Resolution

Improving the resolution of magnetic resonance (MR) image data is critical to computer-aided diagnosis and brain function analysis. Higher resolution helps to capture more detailed content, but typically induces to lower signal-to-noise ratio and longer scanning time. To this end, MR image super-resolution has become a widely-interested topic in recent times. Existing works establish extensive deep models with the conventional architectures based on convolutional neural networks (CNN). In this work, to further advance this research field, we make an early effort to build a Transformer-based MR image super-resolution framework, with careful designs on exploring valuable domain prior knowledge. Specifically, we consider two-fold domain priors including the high-frequency structure prior and the inter-modality context prior, and establish a novel Transformer architecture, called Cross-modality high-frequency Transformer (Cohf-T), to introduce such priors into super-resolving the low-resolution (LR) MR images. Experiments on two datasets indicate that Cohf-T achieves new state-of-the-art performance.

==> figures/attention.tex <==
\begin{figure}
\centering
\includegraphics[width=1\linewidth]{sources/attention9.pdf}
\vspace{-7mm}
\caption{Our devised attention module with inter-head interactions. `LN' stands for layer normalization. `Folding' aggregates features of local patches into patch-level representations. `Unfolding' is the reverse operation of `Folding'. 
%denotes the space-to-depth operation. The reshape operation transforms the input three-dimensional tensor into a two-dimensional tensor by flattening the horizontal and vertical dimensions. 
%Fourier transformation based image adapting~\cite{yang2020fda} is used to transfer source/target images into the target/source domain, which helps to bridge the source and target domain models during the co-training process and make full usage of labeled images. 
%\textcolor{blue}{TODO: add illustration of data distribution before and after applying our cross-domain collaboration.}
}

%\chaowei{change 'image style transfer' to 'image adapting'.}
\label{fig:attention}
\vspace{-6mm}
\end{figure}

==> tables/cmp-ixi.tex <==
\begin{table*}[t]
% \caption{Comparison with existing methods on IXI dataset, under $2\times$, $3\times$, and $4\times$ upsampling settings.}
% \label{tab:ixi}
\centering
\footnotesize
\setlength{\tabcolsep}{2.5mm}{
    \begin{tabular}{l| c|c| c|c |c|c}
        \toprule
        \multirow{2}{*}{Method} & \multicolumn{2}{c|}{4$\times$} & \multicolumn{2}{c|}{3$\times$} & \multicolumn{2}{c}{2$\times$} \\ \cmidrule(l){2-3} \cmidrule(l){4-5} \cmidrule(l){6-7}
                 & PSNR           & SSIM              & PSNR             & SSIM                   & PSNR           & SSIM \\ \midrule
        %Bilinear & 23.93$\pm$1.26 & 0.7360$\pm$0.0293 & 25.66$\pm$1.39   & 0.8134$\pm$0.0238 & 29.60$\pm$1.66 & 0.9136$\pm$0.0148     \\
        \multicolumn{7}{c}{Single Natural Image Super-resolution Methods} \\ \midrule
        Bicubic  & 24.32$\pm$1.28 & 0.7296$\pm$0.0302 & 26.01$\pm$1.40   & 0.8070$\pm$0.0248 & 29.71$\pm$1.68 & 0.9067$\pm$0.0161 \\
        RDN~\cite{zhang2018residual}                       & 29.89$\pm$1.94 & 0.8998$\pm$0.0166 & 31.02$\pm$1.79   & 0.9307$\pm$0.0108 & 33.54$\pm$2.30 & 0.9435$\pm$0.0182 \\
        RCAN~\cite{zhang2018image}                       & 29.60$\pm$1.66 & 0.8936$\pm$0.0148 & 30.79$\pm$1.11   & 0.9302$\pm$0.0194 & 33.66$\pm$1.78 & 0.9422$\pm$0.0231 \\
        SAN~\cite{dai2019second}                       & 29.59$\pm$1.87 & 0.8825$\pm$0.0145 & 31.28$\pm$1.34   & 0.9401$\pm$0.0132 & 34.31$\pm$1.07 & 0.9513$\pm$0.0390 \\
        CFSR~\cite{tian2020coarse} & 29.78$\pm$1.33 & 0.8874$\pm$0.0121 & 31.30$\pm$1.50   & 0.9320$\pm$0.0166 & 34.24$\pm$1.34 & 0.9521$\pm$0.0191 \\
        HAN~\cite{niu2020single}                       & 29.96$\pm$1.57 & 0.8993$\pm$0.0240 & 31.36$\pm$2.00   & 0.9377$\pm$0.0212 & 34.10$\pm$1.89 & 0.9480$\pm$0.0166 \\
        SRResCGAN~\cite{umer2020deep} & 30.24$\pm$1.60 & 0.8924$\pm$0.0155 & 31.21$\pm$1.21   & 0.9388$\pm$0.0198 & 34.02$\pm$1.00 & 0.9522$\pm$0.0150 \\
        SPSR~\cite{ma2020structure}                       & 30.47$\pm$2.33 & 0.8931$\pm$0.0177 & 31.61$\pm$1.88   & 0.9382$\pm$0.0190 & 34.47$\pm$2.13 & 0.9511$\pm$0.0144 \\
        SMSR~\cite{wang2021exploring} & 30.36$\pm$1.88 & 0.9004$\pm$0.0197 & 31.88$\pm$2.01   & 0.9477$\pm$0.0231 & 34.77$\pm$1.81 & 0.9588$\pm$0.0176 \\
        NLSN~\cite{mei2021image} & 30.64$\pm$1.68 & 0.8859$\pm$0.0157 & 31.65$\pm$1.66   & 0.9432$\pm$0.0233 & 34.51$\pm$1.23 & 0.9577$\pm$0.0300 \\
        SwinIR~\cite{liang2021swinir} & 30.91$\pm$2.24 & 0.8915$\pm$0.0226 & 31.83$\pm$1.77   & 0.9385$\pm$0.0271 & 34.62$\pm$1.71 & 0.9401$\pm$0.0271 \\ \midrule
        \multicolumn{7}{c}{Reference-based Natural Image Super-resolution Methods} \\ \midrule
        TTSR~\cite{yang2020learning} & 30.63$\pm$2.31 & 0.9044$\pm$0.0245 & - & - & - & - \\
        MASA-SR~\cite{lu2021masa} & 30.78$\pm$2.07 & 0.9032$\pm$0.0177 & - & - & - & - \\ \midrule
        \multicolumn{7}{c}{MR Image Super-resolution Methods} \\ \midrule
        T2-Net~\cite{feng2021task}                       & 28.99$\pm$2.01 & 0.8604$\pm$0.0142 & 31.07$\pm$2.21   & 0.9313$\pm$0.0155 & 33.31$\pm$1.66 & 0.9441$\pm$0.0134 \\ 
        MTrans~\cite{feng2021mtrans} & 30.01$\pm$2.70 & 0.8729$\pm$0.0233 & 30.45$\pm$1.87   & 0.9298$\pm$0.0201 & 33.92$\pm$1.95 & 0.9471$\pm$0.0140 \\
        MINet~\cite{feng2021multi} & 30.21$\pm$1.86 & 0.8921$\pm$0.0170 & 31.33$\pm$1.90   & 0.9208$\pm$0.0102 & 34.34$\pm$1.99 & 0.9529$\pm$0.0244 \\
        Ours & 31.71$\pm$1.99 & 0.9113$\pm$0.019 & 32.70$\pm$1.58   & 0.9492$\pm$0.0190 & 35.60$\pm$1.615 & 0.9632$\pm$0.0141 \\
        %38.15 &0.9341 &0.9344 &0.9343 &34.14 &0.9212 &0.9234 &0.9245 &31.95 &0.9002 &0.9095 &0.9056  
        %DPSR~\cite{zhang2019deep} & 38.22 &0.9532 &0.9607 &0.9567 &34.55 &0.9389 &0.9321 &0.9356 &32.31 &0.9112 &0.9089 &0.9102  \\
        %MetaSR~\cite{hu2019meta}                    & 38.50 &0.9322 &0.9321 &0.9328 &34.38 &0.9213 &0.9270 &0.9279 &32.37 &0.8835 &0.8295 &0.8313  \\
        %RRIN~\cite{li2020video}                      & 38.04 &0.9752 &0.9788 &0.9787 &34.30 &0.9166 &0.9135 &0.9154 &32.25 &0.9191 &0.9056 &0.9056  \\
        %AdaCoF~\cite{lee2020adacof}                    & 38.46 &0.9758 &0.9772 &0.9777 &35.14 &0.9471 &0.9482 &0.9451 &32.98 &0.9327 &0.9341 &0.9307 \\
        %SAINT~\cite{peng2020saint}                     &38.41 &0.9612 &0.9634 &0.9638 &35.28 &0.9302 &0.9249 &0.9243 &33.15 &0.9078 &0.9135 &0.9014  \\ \midrule
        %PInt-C                     & 38.50 &0.9351 &0.9357 &0.9357 &34.88 &0.9260 &0.9207 &0.9206 &32.26 &0.9076 &0.9229 &0.9239 \\
        %PInt-S                     &38.50   &0.9353  &0.9348  &0.9349  &34.86  &0.9253  &0.9202  &0.9211  &32.26  &0.9054  &0.9225  &0.9228 \\
        %SInt-A                  & 38.75 &0.9440 &0.9431 &0.9453 &34.97 &0.9214 &0.9145 &0.9174 &32.54 &0.9029 &0.8934 &0.8969 \\
        %PInt-C+SInt-A                     &38.76   &0.9521  &0.9519  &0.9523  &35.15  &0.9358  &0.9362  &0.9367  &32.65  &0.9127  &0.9142  &0.9135  \\
        %PInt-S+SInt-A                     &38.73   &0.9529  &0.9517  &0.9521  &35.21  &0.9361  &0.9359  &0.9362  &32.72  &0.9141  &0.9128  &0.9129 \\
        %PInt-C+PInt-S+SInt-A            &38.89   &0.9545  &0.9548  &0.9551  &35.39  &0.9384  &0.9376  &0.9389  &32.85  &0.9166  &0.9159  &0.9158  \\
        %SliceInt-A                  & 38.75 &0.9440 &0.9431 &0.9453 &34.97 &0.9214 &0.9145 &0.9174 &32.54 &0.9029 &0.8934 &0.8969 \\
        %Ours SInt-A & \textbf{39.92} &\textbf{0.9917} &\textbf{0.9936} &\textbf{0.9943} &\textbf{36.75} &\textbf{0.9788} &\textbf{0.9750} &\textbf{0.9786} &\textbf{34.93} &\textbf{0.9599} &\textbf{0.9597} &\textbf{0.9601} \\
        %Ours PInt-C+SInt-A                     &  & & & & & & & & & & & \\
        %Ours PInt-S+SInt-A                     &  & & & & & & & & & & & \\
        %Ours PInt-C+PInt-S+SInt-A            &   &  &  &  & & &  &  &  &  &  & \\
        \bottomrule
    \end{tabular}
}
\caption{Comparison with existing methods on IXI dataset, under $2\times$, $3\times$, and $4\times$ upsampling settings.}
\label{tab:ixi}
\end{table*}
